Theory of Small $x$ Deep Inelastic Scattering NLO Evaluations, and low $Q^2$ Analysis

We calculate structure functions at small $x$ both under the assumption of a hard singularity (a power behaviour $x^{-\lambda}, \lambda$ positive, for $x\rightarrow 0$) or that of a soft-Pomeron dominated behaviour, also called double scaling limit, for the singlet component. A full next to leading order (NLO) analysis is carried for the functions $F_2, F_{\rm Glue}$ and the longitudinal one $F_L$ in $ep$ scattering, and for $x F_3$ in neutrino scattering. The results of the calculations are compared with data (HERA) in the range $x\leq 0.032, 10 gev^2\leq Q^2\leq 1 500 gev^2$. We get reasonable fits, with a chi-squared/d.o.f.$\sim 2$, for both assumptions, but none of them gives a fully satisfactory description. The results improve substantially if combining a soft and a hard component; in this case it is even possible to extend the analysis, phenomenologically, to small values of $Q^2$, $0.31 gev^2\leq Q^2\leq 8.5 gev^2$, and in the $x$ range $6\times10^{-6}\lsim x \lsim 0.04$, with the same hard plus soft Pomeron hypothesis by assuming a saturating expression for the strong coupling, $\tilde{\alpha}_s(Q^2)=4\pi/\beta_0\log[(Q^2+\Lambda_{eff}^2)/\Lambda_{eff}^2]$ The description for low $Q^2$ implies self-consistent values for the parameters in the exponents of $x$. One gets, for the Regge intercepts, $\alpha_{\rho}(0)=0.48$ and $\alpha_P(0)=1.470$ [$\lambda=0.470$], in uncanny agreement with other determinations of these parameters, in particular the results of the large $Q^2$ fits. The fit to is so good that we may look (at large $Q^2$) for signals of a "triple Pomeron" vertex; some evidence is found.

==> changes_in_article <==
%auto-ignore
Changes to ``Theory of small $x$ DIS..." by K. Adel and F. J. Yndur\'ain, No. 
NUCPHB 4778.
\vskip.2cm
1. Two new sections, 5 and 6, with results on the ``hard" plus ``soft" 
Pomeron hypotheses.

2. Corresponding alterations in the Introduction, Sect. 1, and 
Conclusions, Sect. 7.

3. We have removed a few Tables and formulas along the text to lighten it, since
 the main results are now the new ones, Sects. 5, 6.
   

